Numerical Simulation of Microflows using Hermite Spectral Methods

We propose a Hermite spectral method for the spatially inhomogeneous Boltzmann equation. For the inverse-power-law model, we generalize an approximate quadratic collision operator defined in the normalized and dimensionless setting to an operator for arbitrary distribution functions. An efficient algorithm with a fast transform is introduced to discretize this new collision operator. The method is tested for one-dimensional benchmark microflow problems.

==> article_abs_intro.tex <==
% vim: tw=70:spell
\begin{abstract}
A sequence of approximate linear collision models for hard-sphere and
inverse-power-law gases is introduced. These models are obtained by
expanding the linearized Boltzmann collision operator into series, and
a practical algorithm is proposed for evaluating the coefficients in
the series. The sequence is proven to be convergent to the linearized
Boltzmann operator, and it established a connection between the
Shakhov model and the linearized collision model. The convergence is
demonstrated by solving the spatially homogeneous Boltzmann
equation. By observing the magnitudes of the coefficients, simpler
models are developed through removing small entries in the coefficient
matrices.

\vspace*{4mm}
\noindent {\bf Keywords:} linearized collision model, hard sphere,
inverse power law, series expansion
\end{abstract}

\section{Introduction}
The development of high technology requires higher and higher accuracy
in the computer simulation of physical processes. In the numerical
simulation of the Boltzmann equation, people used to focus mainly on
some simplified collision models like BGK, ES-BGK and Shakhov models
\cite{Yang,Mieussens}, while in the recent years, more and more
investigation on the simulation original Boltzmann collision operators
is springing up and some fast methods are proposed
\cite{Mouhot,Gamba,Wu}. The necessity of using the complex collision
models is already clearly stated in these references. However,
currently the fast deterministic methods for simulating complex
collision terms are still restricted to some types of hard spheres,
and the computational cost is still relatively high.

Another type of methods, which also approximates the Boltzmann
equation, is to formulate moment equations from the Boltzmann
equation, and then simulate numerically based on the moment equations
\cite{Struchtrup2003,Torrilhon2006,McDonald}. This method was
introduced by Grad \cite{Grad} and is called the ``moment method''. If
the number of moments is small, the computational cost is much lower
than the direct solver of the Boltzmann equation \cite{Rana}; some
investigation on the use of many moments is also ongoing \cite{NRxx}.
In this direction, people are also starting to concentrate on
collision models other than the simple Maxwell molecules
\cite{Struchtrup2013}. It has been shown in \cite{NRxx,Li} that BGK
and Shakhov collision terms can be easily modelled by the moment
method with almost arbitrary number of moments.  However, the
construction of moment methods with the original collision operator is
obviously not so trivial as the BGK and Shakhov operators
\cite{Truesdell}.

In this paper, we restrict ourselves to the linearized Boltzmann
collision operator. The inconvenience coming from the complex integral
form makes us reconsider those BGK-type models. As is well known, the
inaccuracy of the BGK model lies firstly in its unphysical relaxation
rate of the heat flux, even if the fluid is close to the local
equilibrium. The Shakhov model introduces the Prandtl number, so that
the relaxation rate of the heat flux is physical for near-equilibrium
states. However, higher moments in the Shakhov model just behave the
same as in the BGK model. This is obviously the reason why the Shakhov
model is not accurate enough. If higher moments are considered, more
accurate models may be obtained. In this point of view, the reduction
of the collision model is actually closely related to the moment
method. For example, the BGK collision operator can be considered as a
model which provides the same G10 system (Grad's 10-moment system) as
the linearized Boltzmann collision model, and simply damps other
moments exponentially; similarly, the Shakhov collision operator can
be considered as a model which provides the same G13 system as the
linearized Boltzmann collision model, and damps the other moments
exponentially. In this paper, this idea will be continued to get more
accurate collision models, and naturally, the resulting models can be
regarded as extensions of the BGK and Shakhov models, and they are
especially suitable for the formulation of moment methods.

Grad \cite{Grad} started the moment method from the Hermite expansion
of the distribution function. The moment method is thereby also
regarded as the spectral discretization of the velocity space. Our
discussion will also focus on the spectral expansion of the
distribution function and the linearized collision term. After a brief
introduction of the Boltzmann equation in Section \ref{sec:Boltzmann},
we consider the choice of the spectral basis and the expansion of the
linearized collision term for general collision kernels in Section
\ref{sec:general}. In Section \ref{sec:HS_IPL}, the hard-sphere and
inverse-power-law models are analyzed as two typical applications, and
later, we come back to the construction of approximate collision
models in Section \ref{sec:approx}. Some experiments showing the
quality of the approximation are carried out in Section \ref{sec:exp},
and finally, conclusions are made in Section \ref{sec:conclusion}.


==> article_intro.tex <==
\section{Introduction}
Over a century ago, Boltzmann devised a profound equation describing the
statistical behavior of gas molecules. A number of interesting theoretical and
practical problems emerged due to the birth of this equation, among which the
numerical simulation for this six-dimensional Boltzmann equation is one
significant topic after the invention of computers. The difficulty comes partly
from its high dimensionality, and partly from its complicated integral operator
modeling the binary collision of gas molecules. People have been using the
Monte Carlo method \cite{Bird} to overcome the difficulty caused by high
dimensionality, but nowadays, a six-dimensional simulation using a
deterministic solver is no longer unaffordable due to the fast growth of
computer flops. Fully six-dimensional computations are carried out in
\cite{Xu2012,Dimarco2015} for the simplified BGK-type collision terms. However,
numerical simulation of the original Boltzmann equation with the binary
collision operator still requires a large amount of computational resources
\cite{Dimarco2018}.

Currently, the deterministic discretization of the binary collision operator
can be categorized into three types: the discrete velocity method
\cite{goldstein1989, Panferov2002}, the Fourier spectral method
\cite{Pareschi1996, Hu2017}, and the Hermite spectral method \cite{Grohs2017,
Gamba2018}. The discrete velocity method is hardly used in the numerical
simulation due to its low order of convergence \cite{Panferov2002}, whereas the
Fourier spectral method is more popular because of its fast convergence rate
and high numerical efficiency. Compared with the Fourier spectral method which
requires periodization of the distribution function, the Hermite spectral
method looks more natural since the basis functions with orthogonality in
$\mathbb{R}^3$ are employed. In fact, the Hermite spectral method has a longer
history and has been known as the moment method since Grad's work \cite{Grad}.
Grad proposed in \cite{Grad} a general method to find the expansion of the
binary collision term with Hermite basis functions. Later, a similar way to
expand the binary collision term using Sonine polynomials (also known as
spherical Hermite polynomials) was proposed in \cite{Kumar}. The techniques
used in formulating the expansion are also introduced in the book
\cite{Truesdell}.

Despite these works, the Hermite spectral method is used in the numerical
simulation only until recently \cite{Grohs2017, Gamba2018}. There are two
major difficulties in applying this method: one is the evaluation of the
coefficients in the expansion of the collision operator; the other is the huge
computational cost due to its quadratic form. Although the general procedure to
obtain the coefficients is given in \cite{Grad, Truesdell}, following such a
procedure involves expansion of a large number of huge polynomials, which is
quite expensive even for a modern computer algebraic system; Kumar \cite{Kumar}
provided a formula in his expansion using Sonine polynomials, while the formula
involves evaluation of a large number of Talmi coefficients, which is not
tractable either. As for the computational cost, the computational time of one
evaluation of the collision operator is proportional to the cube of the number
of degrees of freedom, while in the Fourier spectral method, the time
complexity for a direct Galerkin discretization is only the square of the
number of modes.

This work is devoted to both of the aforementioned issues. On one hand, by
using a number of properties for relavant polynomials, we provide explicit
formulas for all the coefficients appearing in the expansion of the collision
operator with the Hermite spectral method. These formulas are immediately
applicable in the sense of coding, and the computational cost is affordable for
a moderate number of degrees of freedom. On the other hand, we combine the
modeling strategy and the numerical technique to form a new way to discretize
the collision term, where only a portion in the truncated series expansion is
treated ``quadratically'', and the remaining part just decays exponentially
as in the BGK model. Thus the computational cost is greatly reduced and we can
still capture the evolution of low-order moments accurately.

The rest of this paper is organized as follows. In Section \ref{sec:Bol_Her},
we briefly review the Boltzmann equation and the Hermite expansion of the
distribution function. In Section \ref{sec:general}, we first give an explicit
expression for the series expansion of the quadratic collision operator, and
then construct approximate collision models based on such an expansion. Some
numerical experiments verifying our method are carried out in Section
\ref{sec:numerical} and some concluding remarks are made in Section
\ref{sec:conclusion}. Detailed derivation of the expansion is given in the
Appendix.

